Latin American HECAP Physics Briefing Book

For the first time the scientific community in Latin America working at the forefront of research in high energy, cosmology and astroparticle physics (HECAP) have come together to discuss and provide scientific input towards the development of a regional strategy. The present document, the Latin American HECAP Physics Briefing Book, is the result of this ambitious bottom-up effort. This report contains the work performed by the Preparatory Group to synthesize the main contributions and discussions for each of the topical working groups. This briefing book discusses the relevant emerging projects developing in the region and considers potentially impactful future initiatives and participation of the Latin American HECAP community in international flagship projects to provide the essential input for the creation of a long-term HECAP strategy in the region.

==> astro/Makefile <==
#makefile

IMAGEDIR    := figures
USEPDFLATEX := 1

##########################################################

DEPENDENCIES := $(addsuffix .tex, $(shell grep -h --extended-regexp --regexp='^\\input{.*}' *.tex | grep -v latex | sed -E 's/^\\input\{|\}//g')) ref.bib
ifdef IMAGEDIR
  DEPENDENCIES += $(shell find $(IMAGEDIR) -type f | grep -v /.svn/)
endif

.PHONY: all clean #authors
 
all: astro3.pdf 
	
clean:
	for e in .tex~ .ps .pdf .dvi .log .aux .bbl .blg .out .spl .toc; do test -f astro3$$e && rm astro3$$e;  done; exit 0

# general rules
%.pdf: %.tex $(DEPENDENCIES)
	pdflatex --shell-escape $<
	bibtex $*
	for i in 1 2 3; do \
	  pdflatex --shell-escape $<  |  \
		  awk '/^LaTeX Warning:/||/natbib Warning:/{f=1;w=w$$0"\n";print;next}{print}END{if(f)print "\n\033[31;1mWarning summary:\n\033[0;33m"w"\033[0m";exit !f}' || \
	  exit 0; \
	done	


==> astro/preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Template for lab reports used at BIT modified from STIMA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Loading packages that alter the style
\usepackage[]{graphicx}
\graphicspath{{figures/}}
\usepackage[]{color}
\usepackage{alltt}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{mathptmx}

\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}
\setlength{\parskip}{\smallskipamount}
\setlength{\parindent}{12pt}

% Set page margins
\usepackage[top=60pt,bottom=60pt,left=78pt,right=78pt]{geometry}
\usepackage{subcaption}
% Package used for placeholder text
\usepackage{lipsum}
\usepackage{booktabs}
\usepackage{multirow}
% Prevents LaTeX from filling out a page to the bottom
\raggedbottom

% Adding both languages
\usepackage[english]{babel}

% All page numbers positioned at the bottom of the page
\usepackage{fancyhdr}
\fancyhf{} % clear all header and footers
\fancyfoot[C]{\thepage}
\renewcommand{\headrulewidth}{0pt} % remove the header rule
\pagestyle{fancy}

% Changes the style of chapter headings
\usepackage{titlesec}
\titleformat{\chapter}
   {\normalfont\LARGE\bfseries}{\thechapter.}{1em}{}
% Change distance between chapter header and text
\titlespacing{\chapter}{0pt}{40pt}{2\baselineskip}

% Adds table captions above the table per default
\usepackage{float}
\floatstyle{plaintop}
\restylefloat{table}

% Adds space between caption and table
\usepackage[tableposition=top]{caption}

% add cc license
\usepackage[
type={CC},
modifier={by-nc-sa},
version={4.0},
]{doclicense}

% Adds hyperlinks to references and ToC
\usepackage{hyperref}
% Uncomment the line below this block to set all hyperlink color to black
\hypersetup{
	colorlinks,
	linkcolor={blue},
	citecolor={green!90!black},
	urlcolor={red!70!black}
}
%\hypersetup{hidelinks,linkcolor = black} % Changes the link color to black and hides the hideous red border that usually is created

% Set specific color for hyperref
\usepackage{xcolor}


% tcolorbox; Notice! add "-shell-escape" to the compile command
\usepackage{tcolorbox}



% Separates the first part of the report/thesis in Roman numerals
\frontmatter

